Boundary topological entanglement entropy in two and three dimensions

The topological entanglement entropy is used to measure long-range quantum correlations in the ground state of topological phases. Here we obtain closed form expressions for topological entropy of (2+1)- and (3+1)-dimensional loop gas models, both in the bulk and at their boundaries, in terms of the data of their input fusion categories and algebra objects. Central to the formulation of our results are generalized $\mathcal{S}$-matrices. We conjecture a general property of these $\mathcal{S}$-matrices, with proofs provided in many special cases. This includes constructive proofs for categories up to rank 5.

==> sections/preamble.tex <==
% !TeX spellcheck = en_US
% This line sets the project root file.
% !TEX root = ../WW_EntanglementEntropy.tex
%

\makeatletter
\newcommand\orcid[1]
{
	\@AF@join{\href{https://orcid.org/#1}{ORCID:#1}}%
}%

\newcommand\commoncomment[1]
{
	\collaboration{#1}
}%

\def\@homepage#1#2{%
	\endgroup
	\@AF@join{#1\href{https://#2}{#2}}%
}%

\makeatother

\usepackage[utf8]{inputenc}

\usepackage[english]{babel}
\makeatletter\AtBeginDocument{\let\@elt\relax}\makeatother %Workaround to fix error in babel package


\usepackage[export]{adjustbox}
\usepackage[table]{xcolor}
\usepackage{booktabs}
\usepackage{physics}
\usepackage{amsmath,dsfont,amsfonts,mathtools,slashed,amssymb}
\usepackage[breaklinks]{hyperref}
\usepackage{array,multirow}
\usepackage{bm}
\usepackage{lipsum}
\usepackage{mathrsfs}
\usepackage[capitalise]{cleveref}
\usepackage{enumerate}
\usepackage{setspace}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{amsthm}
\usepackage{color}
\usepackage{import}
\usepackage{lipsum}
\usepackage{xfrac}
\usepackage{kbordermatrix}
\usepackage{thmtools}
\usepackage{etoolbox}
\usepackage[normalem]{ulem}
\usepackage{amsmath}

\usepackage{apptools}
\AtAppendix{
	\numberwithin{lemma}{section}
	\numberwithin{claim}{section}
	\numberwithin{definition}{section}
	\numberwithin{corollary}{section}
}

\usepackage[font=small,labelfont=bf,textfont=normalfont,singlelinecheck=off,justification=raggedright]{caption}
\usepackage[font=small,labelfont=bf,textfont=normalfont,singlelinecheck=off,justification=raggedright]{subcaption}

\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{darkblue}{RGB}{0,0,127}
\definecolor{darkgreen}{RGB}{5,180,50}
\definecolor{darkred}{RGB}{200, 10, 42}

\definecolor{nicegreen}{RGB}{20, 200, 20}

\usepackage{pgfplots}

% Tikz thinkgs
\pgfplotsset{compat=newest}
\usetikzlibrary{external}

\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
{ \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }

\usetikzlibrary{backgrounds,fit,decorations.pathreplacing,calc,calligraphy,shapes.misc,decorations.pathmorphing,arrows,decorations.pathmorphing,backgrounds,positioning,fit,calc,patterns,shapes,decorations.markings,shadings}

\tikzstyle{inline text}=[text height=1.1ex, text depth=0.1ex, yshift=-.1ex]
\newcommand{\trivalentvertex}[4]{
	\draw (0,0)--(0,1);
	\node[above,inline text] at (0,1) {#1};
	\draw (0,0)--(-0.707,-0.707);
	\node[below,inline text] at (-0.707,-0.707) {#2};
	\draw (0,0)--(0.707,-0.707);
	\node[below,inline text] at (0.707,-0.707) {#3};
	\node[left,inline text] at (0,0) {#4};
}


%% Externalizing should now work automatically
\ifthenelse{\equal{\tikzexternalcheckshellescape}{}}{}{
	\tikzexternalize[prefix=figures/]
	\tikzset{external/system call={
				if [ -x "$(command -v pdflatex)" ]; then
				pdflatex \tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname "\image" "\texsource";rm  -f "\image".log ; rm -f "\image".dpth ; rm  -f "\image"Notes.bib; rm  -f "\image".md5;
				else
				/usr/local/texlive/2018/bin/x86_64-darwin/pdflatex \tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname "\image" "\texsource";rm "\image".log && rm "\image".dpth && rm "\image"Notes.bib;
				fi;
			}}
}

%%%%%%%%%%%%%%%%
\newcommand{\includeTikz}[2]
{
	\tikzifexternalizing
	{
		\includeTikzrm{#1}{#2}
	}
	{
		\IfFileExists{figures/#1.pdf}{
			\includegraphics{figures/#1}
		}
		{
			\includeTikzrm{#1}{#2}
		}
	}
}

\newcommand{\includeTikzrm}[2]{
	\tikzset{external/remake next}
	\tikzsetnextfilename{#1}
	#2
}

% Href

\hypersetup{
	colorlinks,
	linkcolor=darkred,
	citecolor=darkblue,
	filecolor=darkred,
	urlcolor=darkblue,
	pdftitle={Topological entropy at the boundary},
	pdfauthor={Jacob C. Bridgeman, Benjamin J. Brown, Samuel J. Elman}
}

% Math operators
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\N}{\mathcal{N}}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\ob}{ob}

\newcommand{\Umat}{\mathcal{U}}
\newcommand{\Smat}{\mathcal{S}}
\newcommand{\stab}{\mathcal{G}}
\newcommand{\Tmat}{\mathcal{T}}
\DeclareMathOperator{\rka}{rk}
\newcommand{\rk}[1]{\rka(#1)}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}
\newcommand{\transpose}{\mathbf{T}}

\newcommand\one{\boldsymbol{1}}

\newcommand{\ZZ}[1]{\mathbb{Z}_{#1}}

\newcommand{\dual}[1]{\bar{#1}}

\newcommand{\vvec}[1]
{
	\operatorname{\bf Vec}
	\ifstrequal{#1}{}
	{}
	{\left(#1\right)}
}

\newcommand{\rrep}[1]
{
	\operatorname{\bf Rep}
	\ifstrequal{#1}{}
	{}
	{\left(#1\right)}
}

\newcommand{\vvectwist}[2]
{
	\operatorname{\bf Vec}^{#2}
	\ifstrequal{#1}{}
	{}
	{\left(#1\right)}
}

\newcommand{\set}[2]{
	\left\{#1
	\ifthenelse{\equal{#2}{}}{}{\,\middle|\,#2}
	\right\}
}

\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\DeclareMathOperator{\id}{id}

\DeclareMathOperator{\rev}{op}

\newcommand{\C}{\mathcal{C}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\cat}[1]{\mathcal{#1}}
\newcommand{\comp}[1]{{#1}^{c}}

\newcommand{\mug}[1]{
	\mathchoice{\mathcal{Z}_2\!\left(#1\right)}
	{\mathcal{Z}_2\!\left(#1\right)}
	{\mathcal{Z}_2\left(#1\right)}
	{\mathcal{Z}_2\left(#1\right)}
}

\newcommand{\drinfeld}[1]{
	\mathchoice{\mathcal{Z}\!\left(#1\right)}
	{\mathcal{Z}\!\left(#1\right)}
	{\mathcal{Z}\left(#1\right)}
	{\mathcal{Z}\left(#1\right)}
}

\newcommand{\indicator}[1]{
	\delta_{#1}
}


% Theorem styles

\declaretheorem[mdframed={linecolor=black!10,linewidth=1pt,
			leftmargin=-5pt,rightmargin=-5pt,
			innerleftmargin=5pt,innerrightmargin=5pt,
			innertopmargin=-2pt,
			innerbottommargin=5pt},name=Theorem,Refname={Theorem,Theorems}]{thm}

\declaretheorem[mdframed={linecolor=black!10,linewidth=1pt,
			leftmargin=-5pt,rightmargin=-5pt,
			innerleftmargin=5pt,innerrightmargin=5pt,
			innertopmargin=-2pt,
			innerbottommargin=5pt},name=Conjecture,Refname={Conjecture,Conjectures}]{conjecture}

\declaretheorem[mdframed={linecolor=black!10,linewidth=1pt,
			leftmargin=-5pt,rightmargin=-5pt,
			innerleftmargin=5pt,innerrightmargin=5pt,
			innertopmargin=-2pt,
			innerbottommargin=5pt},name=Corollary,Refname={Corollary,Corollaries}]{cor}

\newtheorem{corollary}[cor]{Corollary}
\crefname{corapp}{Corollary}{Corollaries}

\declaretheorem[name=Claim,Refname={Claim,Claims}]{claim}

\declaretheorem[name=Lemma,Refname={Lemma,Lemmas}]{lemma}

\declaretheorem[name=Example,Refname={Example,Examples}]{example}

\newtheorem*{examples*}{Examples}

\declaretheorem[name=Definition,Refname={Definition,Definitions}]{definition}

\newtheoremstyle{TheoremNum}
{\topsep}{\topsep}              %%% space between body and thm
{\itshape}                      %%% Thm body font
{}                              %%% Indent amount (empty = no indent)
{\bfseries}                     %%% Thm head font
{.}                             %%% Punctuation after thm head
{ }                             %%% Space after thm head
{\thmname{#1}\thmnote{ \bfseries #3}}%%% Thm head spec
\theoremstyle{TheoremNum}

\newtheorem{thm_rep}{Theorem}
\newtheorem{corollary_rep}{Corollary}
\newtheorem{lemma_rep}{Lemma}
\newtheorem{claim_rep}{Claim}


% Citation formatting
\let\oldonlinecite\onlinecite
\renewcommand{\onlinecite}[1]{Ref.~\oldonlinecite{#1}}

\newcommand{\onlinecites}[1]{Refs.~\oldonlinecite{#1}}

\newcommand{\creflastconjunction}{, and~}

% Table formatting
\usepackage[]{threeparttable}
\let\oldtnote\tnote
\renewcommand{\tnote}[1]{\hyperref[tnote:#1]{\oldtnote{#1}}}
\renewcommand{\TPTnoteLabel}[1]{\label{tnote:#1}\oldtnote{#1}}

\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}

\newcommand{\greycline}[1]{\arrayrulecolor[gray]{.8}\cline{#1}\arrayrulecolor{black}}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}

% Style choices to make
\let\define\uline

\newcommand{\LWTEE}{\gamma}
\newcommand{\LWbndTEE}{\Gamma}

\newcommand{\WWTEE}{\delta}

\newcommand{\WWbndTEELoop}{\Delta_{\circ}}
\newcommand{\WWbndTEEPoint}{\Delta_{\bullet}}

\renewcommand{\FR}[4]{\mathrm{FR}^{#1,#2}_{#3;#4}}
\usepackage{pifont}
